Accelerating the Distributed Kaczmarz Algorithm by Strong Over-relaxation

The distributed Kaczmarz algorithm is an adaptation of the standard Kaczmarz algorithm to the situation in which data is distributed throughout a network represented by a tree. We isolate substructures of the network and study convergence of the distributed Kazmarz algorithm for relatively large relaxation parameters associated to these substructures. If the system is consistent, then the algorithm converges to the solution of minimal norm; however, if the system is inconsistent, then the algorithm converges to an approximated least-squares solution that is dependent on the parameters and the network topology. We show that the relaxation parameters may be larger than the standard upper-bound in literature in this context and provide numerical experiments to support our results.

==> DAGs.tex <==
\section{Non-tree structures}

Suppose the distributed system of equations is in the form of a directed acyclic graph (DAG) instead of a tree. We can represent this by a partial order $\preceq$ on the nodes. We write $u\prec v$ when $u\preceq v$ and $u\ne v$. We add a directed edge $(u,v)$ to the edge set $E$ whenever $u\prec v$, and when there is no $w$ such that $u\prec w\prec v$. When there is such a $w$, the corresponding edge can only decrease the rate of convergence, so we remove it. If $(u,v)\in E$, we denote this by $u<v$ or $v>u$. The resulting graph $G=(V,E)$ is the DAG of interest. We assume $G$ is a weakly connected graph. That is, the undirected graph is connected.

Let there be $s$ minimal nodes $r_1,\dots,r_s$ and $t$ maximal nodes $\ell_1,\dots,\ell_t$. For any edge $(u,v)$, we assign dispersion and pooling weights $w_d(u,v)$ and $w_p(u,v)$. We require the weights to be assigned such that for each node $u$ that isn't maximal: \[
\sum_{v>u}w_p(u,v)=1
\] and for each node $u$ that isn't minimal:
\[
\sum_{v<u}w_d(v,u)=1.
\]
In the beginning of an iteration, each minimal node $r_i$ starts with an estimate $\vec{x}_{r_i}^{(n)}$. Then, iterating in a topological order on the nodes, we disperse by the following Kaczmarz update:
\begin{align*}
\vec{z}_v^{(n)}&=\sum_{(u,v)\in E} w_d(u,v)\vec{x}_u^{(n)}\\
\vec{x}_v^{(n)}&=\vec{z}_v^{(n)}+\omega_v\frac{b_v-S_v\vec{z}_v^{(n)}}{\lVert \vec{a}_v\rVert^2}\vec{a}_v .
\end{align*}

We set $y_v^{(n)}=x_v^{(n)}$ for each maximal node $v$. Then, in a reverse topological order, we pool in the following update:
\[
\vec{y}_u^{(n)}=\sum_{(u,v)\in E}w_p(u,v)\vec{y}_v^{(n)}.
\]

At the end of the iteration, we set $\vec{x}_{r_i}^{(n+1)}=\vec{y}_{r_i}^{(n)}$ for each minimal node $r_i$.

\begin{figure}[!h]
    \centering
\begin{tikzpicture}    
    
\def\w{1.0}
\def\u{0.50}

\node[circle,fill=white!20!white] (0) at (-3*\w,1*\u){};
\node[circle,fill=teal!20!white] (1) at (-3*\w,0*\u){1};
\node[circle,fill=teal!20!white] (2) at (-1*\w,0*\u){2};
\node[circle,fill=teal!20!white] (3) at (-4*\w,-2*\u){3};
\node[circle,fill=teal!20!white] (4) at (-2*\w,-2*\u){4};
\node[circle,fill=teal!20!white] (5) at (-5*\w,-4*\u){5};
\node[circle,fill=teal!20!white] (6) at (-3*\w,-4*\u){6};


\draw[->,thick] (1) to (3);
\draw[->,thick] (1) to (4);
\draw[->,thick] (2) to (4);
\draw[->,thick] (3) to (5);
\draw[->,thick] (3) to (6);
\draw[->,thick] (4) to (6);

\node[circle,fill=red!20!white] (1a) at (1*\w,0*\u){1};
\node[circle,fill=red!20!white] (2a) at (2*\w,-2*\u){2};
\node[circle,fill=red!20!white] (3a) at (1*\w,-4*\u){3};
\node[red] (4a) at (1*\w,-2*\u){\huge{$\times$}};

\draw[->,thick] (1a) to (2a);
\draw[->,thick] (1a) to (3a);
\draw[->,thick] (2a) to (3a);


\end{tikzpicture}    
\caption{An example of a DAG (left), and an example of an arrow we do not include (right)}
\label{fig:DFS DAGS}
\end{figure}

\subsection{Notation}
For each node $v$, we let $P_v$ be the linear projection onto $\mathcal{N}(S_v)$, and $Q_v$ be the affine projection onto the linear manifold $S_v(\vec{z})=b_v$, just as it was for trees.

For any two (not necessarily distinct) minimal nodes $r_{m_1}$ and $r_{m_2}$, let there be $p(m_1,m_2)$ paths of the form
\[
\mathscr{P}_{m_1,m_2,i}:v_1<v_2<\cdots<v_j>\cdots>v_{k-1}> v_k
\]

where $v_1=r_{m_1}$, $v_k=r_{m_2}$, and $v_j$ is a maximal node. These paths tell us how two minimal nodes communicate in one iteration. In fact, there is a notion of the distance between two minimal nodes based on how many such paths are required to get from one node to the other. This is illustrated in Figure~\ref{fig:rootdistance}. Let $d$ denote the maximum distance between any two minimal nodes. If there is only one minimal node we let $d=1$. For each such path we assign the matrix
\[
P(\mathscr{P}_{m_1,m_2,i})=w_d(v_1,v_2)\cdots w_d(v_{j-1},v_j)w_p(v_{j+1},v_j)\cdots w_p(v_k,v_{k-1})P_{v_j}\cdots P_{v_1}.
\]

\begin{figure}
    \centering
\begin{tikzpicture}
    
\def\w{1.0}
\def\u{0.5}

\node[circle,fill=teal!20!white,minimum size =0.7cm] (1) at (-8*\w,0*\u) {$r_1$};
\node[circle,fill=teal!20!white,minimum size =0.7cm] (2) at (-6*\w,0*\u) {$r_2$};
\node[circle,fill=teal!20!white,minimum size =0.7cm] (3) at (-4*\w,0*\u) {$r_3$};
\node[circle,fill=teal!20!white,minimum size =0.7cm] (4) at (-2*\w,0*\u) {$r_4$};
\node[circle,fill=teal!20!white,minimum size =0.7cm] (5) at (-7*\w,-2*\u) {};
\node[circle,fill=teal!20!white,minimum size =0.7cm] (6) at (-5*\w,-2*\u) {};
\node[circle,fill=teal!20!white,minimum size =0.7cm] (7) at (-3*\w,-2*\u) {};
\node[circle,fill=teal!20!white,minimum size =0.7cm] (8) at (-6*\w,-4*\u) {};

\draw[->,thick] (1) to (5);
\draw[->,thick] (5) to (8);
\draw[->,thick] (2) to (5);
\draw[->,thick] (3) to (6);
\draw[->,thick] (3) to (7);
\draw[->,thick] (4) to (7);
\draw[->,thick] (5) to (8);
\draw[->,thick] (6) to (8);

\node[circle,fill=red!20!white,minimum size =0.7cm] (1b) at (0*\w,0*\u) {$r_1$};
\node[circle,fill=red!20!white,minimum size =0.7cm] (2b) at (1.5*\w,-2*\u) {$r_3$};
\node[circle,fill=red!20!white,minimum size =0.7cm] (3b) at (0*\w,-4*\u) {$r_2$};
\node[circle,fill=red!20!white,minimum size =0.7cm] (4b) at (3.5*\w,-2*\u) {$r_4$};

\draw[-,thick] (1b) to (2b);
\draw[-,thick] (1b) to (3b);
\draw[-,thick] (2b) to (3b);
\draw[-,thick] (2b) to (4b);

\end{tikzpicture}
    \caption{A DAG (left) and the distance graph of the minimal nodes (right). The diameter $d=2$ in this example.}
    \label{fig:rootdistance}
\end{figure}

\subsection{Consistent Systems}

Now, we build an $s\times s$ block matrix $\mathcal{P}$ with blocks of size $n\times n$. Let $\mathcal{P}_j$ denote the $j$th row of blocks and $\mathcal{P}_{j,i}$ denotes the block in row $j$ and column $i$. Then we define
\[
\mathcal{P}_{j,i}=\sum_{k=1}^{p(i,j)}P(\mathscr{P}_{i,j,k}).
\]

If $\vec{x}$ is the unique solution to the system $A\vec{x}=b$ orthogonal to $\mathcal{N}(A)$, then one iteration can be expressed in the following way.
\begin{align*}
\vec{x}'&=\begin{pmatrix}\vec{x}^T&\cdots&\vec{x}^T\end{pmatrix}^T\\
\vec{x}^{(n)}&=\begin{pmatrix}\left(\vec{x}_{r_1}^{(n)}\right)^T&\cdots &\left(\vec{x}_{r_s}^{(n)}\right)^T\end{pmatrix}^T\\
\vec{x}^{(n+1)}&=\vec{x}'-\mathcal{P}\left(\vec{x}'-\vec{x}^{(n)}\right)=:\mathcal{Q}(\vec{x}^{(n)})
\end{align*}

In order to prove convergence to the minimum norm solution, we make use of the following norm on $\mathbb{C}^{ns}$.
\[
\lVert \vec{x}\rVert_\infty:=\max\{\lVert\vec{x}_1\rVert,\dots,\lVert\vec{x}_s\rVert\}
\]

Let $U=\mathrm{span}(\vec{a}_1,\dots,\vec{a}_m)$, and
\[
W=\left\{ \begin{pmatrix}\vec{v}^T&\cdots&\vec{v}^T\end{pmatrix}^T\in \mathbb{C}^{ns}\mid \vec{v}\in U^\perp\right\}.
\]

See Figure~\ref{fig:venndiagram}.

\begin{figure}
\centering
\begin{tikzpicture}
\draw (-4, -2.5) rectangle (4, 3);
\draw (-1.5, 0) circle (2);
\draw (1.5, 0) circle (2);
\draw (-1.75, -0.5) circle (0.75);
\draw (1.75, -0.5) circle (0.75);

\node at (0, 2.5) (A) {$\mathbb{C}^{ns}$};
\node at (-1.5, 1) (B) {$(U^\perp)^s$};
\node at (1.5, 1) (C) {$W^\perp$};
\node at (-1.75, -0.5) (D) {$W$};
\node at (1.75, -0.5) (E) {$U^s$};
\end{tikzpicture}
\caption{A Venn Diagram showing the relationships between the various subspaces. We draw two subspaces as disjoint if they only share the zero vector.}
\label{fig:venndiagram}
\end{figure}

\begin{lemma}
\label{lma:KidentityonW}
If $\vec{w}\in W$, then $\mathcal{P}\vec{w}=\vec{w}$.
\end{lemma}

\begin{proof}
Since $\vec{w}\in W$, the initial estimates at each root are all equal to some vector $
\vec{v}\in V^\perp$. Then these estimates remain unchanged at each node in both dispersion and pooling. In particular, the resulting estimates at the roots remain unchanged, therefore $\mathcal{P}\vec{v}=\vec{v}$.
\end{proof}

\begin{lemma}
\label{lma:normKleq1}
$\lVert \mathcal{P}\rVert_\infty \le 1$.
\end{lemma}

\begin{proof}
Let $\lVert \vec{z}\rVert_\infty=1$. Due to the restrictions on dispersion and pooling weights, and since $\lVert P_v\rVert\le 1$ for any $v$, we have 
\begin{equation}
\label{eqn:SumKlt1}
\sum_{i=1}^{s}\lVert \mathcal{P}_{j,1}\rVert\le 1.
\end{equation}

In fact, equality holds if there are multiple solutions. If $\vec{x}_{i}$ denotes the $i$th $n$-sized block of a vector $\vec{x}$, then we have $\lVert \vec{z}_i\rVert\le 1$ for all $i$ since $\lVert\vec{z}\rVert_\infty =1$. For each $i$ we must also have
\begin{align*}
\lVert(\mathcal{P}\vec{z})_i\rVert&=\lVert \mathcal{P}_{i,1}\vec{z}_1+\cdots+\mathcal{P}_{i,s}\vec{z}_s\rVert\\
&\le \lVert \mathcal{P}_{i,1}\vec{z}_1\rVert+\cdots+\lVert \mathcal{P}_{i,s}\vec{z}_s\rVert\\
&\le 1
\end{align*}

Since every block of $\mathcal{P}\vec{z}$ has norm at most $1$ for any unit vector $\vec{z}$, it holds that $\lVert \mathcal{P}\rVert_\infty \le 1$.
\end{proof}

\begin{lemma}
\label{lma:KpreservesWperp}
$\mathcal{P}(U^s)\subseteq U^s$
\end{lemma}

\begin{proof}
The blocks of $\mathcal{P}$ are formed from weighted averages of products of the matrices $P_v$, each of which preserves $U$. Therefore, $\mathcal{P}$ preserves $U^s$

%The subspace $(U^\perp)^s$ is also preserved by $\mathcal{P}$, and it is not hard to show that $\mathcal{P}$ is a self-adjoint operator when restricted to $(U^\perp)^s$. Then it holds that $\mathcal{P}$ preserves $W^\perp\cap (U^\perp)^s$. In fact, let $\vec{w}\in W^\perp \cap(U^\perp)^s$ and $\vec{v}\in W$. Note that $\vec{v}\in (U^\perp)^s$ since $W\le (U^\perp)^s$. Then we have
%\[
%\langle \mathcal{P}\vec{w},\vec{v}\rangle=\langle \vec{w},\mathcal{P}\vec{v}\rangle=\langle \vec{w},\vec{v}\rangle=0
%\]

%since $\vec{w}\in W^\perp$ and $\vec{v}\in W$. Therefore, $\mathcal{P}\vec{w}\in W^\perp\cap (U^\perp)^s$.
\end{proof}

\begin{lemma}
\label{lma:rhoKlt1}
There is an $\alpha<1$ such that for any $\vec{z}\in W^\perp$ we have \[\left\lVert\mathcal{P}^d\vec{z}\right\rVert_\infty\le \alpha\lVert \vec{z}\rVert.\]
\end{lemma}

\begin{proof}
Assume by way of contradiction that there is a unit vector $\vec{z}\in W^\perp$ such that $\lVert \mathcal{P}^{d}\vec{z}\rVert_\infty =1$. By Lemma~\ref{lma:normKleq1}, we have
\[
\lVert\mathcal{P}^m \vec{z}\rVert_\infty =1
\]

for any $0<m\le d$. Since $\lVert \mathcal{P}^{d}\vec{z}\rVert_\infty=1$, we know $\lVert (\mathcal{P}^{d}\vec{z})_i\rVert=1$ for some $i$. Then we have
\begin{align*}
1=\left\lVert (\mathcal{P}^{d}\vec{z})_i\right\rVert&=\left\lVert (\mathcal{P}(\mathcal{P}^{d-1}\vec{z}))_i\right\rVert\\
&= \left\lVert \mathcal{P}_{i,1}(\mathcal{P}^{d-1}\vec{z})_1+\cdots+\mathcal{P}_{i,s}(\mathcal{P}^{d-1}\vec{z})_s\right\rVert\\
&\le \lVert \mathcal{P}_{i,1}\rVert+\cdots+\lVert \mathcal{P}_{i,s}\rVert\tag{1}\\
&\le 1.
\end{align*}

Therefore the inequality in (1) is strictly equal. From (1), we see that
\[\left\lVert \mathcal{P}_{i,j}\left(\mathcal{P}^{d-1}\vec{z}\right)_j\right\rVert=\lVert \mathcal{P}_{i,j}\rVert\]

for each $1\le j\le s$ when $\mathcal{P}_{i,j}\ne 0$. Therefore, $\left \lVert\left ( \mathcal{P}^{d-1}\vec{z}\right)_j \right \rVert =1$ and $\left ( \mathcal{P}^{d-1}\vec{z} \right )_j$ is a fixed point of $P_v$ for each node $v\succeq r_i$ on any such path $P_{i,j,k}$. By repeating this argument $d$ times, we see that for all $1\le i\le s$, $\lVert\vec{z}_i\rVert=1$ and $\vec{z}_i$ is a fixed point of $P_v$ for all nodes $v\succeq r_i$. Then
\begin{align*}
1=\lVert (\mathcal{P}\vec{z})_i\rVert&=\lVert \mathcal{P}_{i,1}\vec{z}_1+\cdots+\mathcal{P}_{i,s}\vec{z}_s\rVert\\
&=\left\lVert \lVert \mathcal{P}_{i,1}\rVert \vec{z}_1+\cdots+\lVert \mathcal{P}_{i,s}\rVert \vec{z}_s\right\rVert\\
&\le \lVert \mathcal{P}_{i,1}\rVert \lVert \vec{z}_1\rVert+\cdots+\lVert \mathcal{P}_{i,s}\rVert \lVert\vec{z}_s\rVert\tag{2}\\
&=\lVert \mathcal{P}_{i,1}\rVert+\cdots+\lVert \mathcal{P}_{i,s}\rVert\\
&\le 1.
\end{align*}

Therefore we have strict equality in (2), which can only happen when
\[\lVert \mathcal{P}_{i,1}\rVert \vec{z}_1,\dots, \lVert\mathcal{P}_{i,s}\rVert \vec{z}_s\] are parallel vectors. So whenever there is a path from $r_i$ to $r_j$, we have $\mathcal{P}_{i,i}$ and $\mathcal{P}_{i,j}$ are nonzero, thus $\vec{z}_i=\vec{z}_j$. And since there is a sequence of paths between any two minimal nodes $r_i$ and $r_j$, we have that all blocks of $\vec{z}$ are equal. Therefore, each block of $\vec{z}$ is the same fixed point of $P_v$ for all nodes $v$. But this can only happen if $\vec{z}\in W\cap W^\perp=\{\vec{0}\}$. This contradicts the fact that $\lVert \vec{z}\rVert_\infty=1$, so the statement holds for
\[
\alpha=\max_{\vec{z}\in W^\perp,\ \vec{z}\ne \vec{0}}\left \{\frac{\lVert \mathcal{P}^d\vec{z}\rVert_\infty}{\lVert \vec{z}\rVert_\infty}\right\}<1.
\]
\end{proof}

\begin{lemma}
\label{lma:sequence_zk_dags}
There is a sufficiently large integer $j$ such that for any sequence $\{\vec{z}_k\}$ in $W\oplus U^s$ with
\[
\lVert \vec{z}_k\rVert\le 1,\quad \lim_{k\to\infty}\lVert \mathcal{P}^j\vec{z}_k\rVert=1.
\]

it holds that
\[
\lim_{k\to\infty}(I-\mathcal{P}^j)\vec{z}_k=\vec{0}.
\]
\end{lemma}

\begin{proof}
Let $\mathcal{H}_1=W$ and apply Lemma~\ref{Lemma3.3} on the operator $\mathcal{P}^j$ using Lemmas~\ref{lma:KidentityonW}, \ref{lma:KpreservesWperp} and \ref{lma:rhoKlt1}. Note that Lemma~\ref{lma:rhoKlt1} implies that $\rho(\mathcal{P}|_{U^s})<1$ and therefore $\lVert \mathcal{P}^j|_{U^s}\rVert<1$ for a sufficiently large $j$ by Gelfand's formula.
\end{proof}

\begin{lemma}
\label{lma:nullspace_IminusK}
$\mathcal{N}(I-\mathcal{P})\cap \left(W\oplus U^s\right)=W$
\end{lemma}

\begin{proof}
Suppose $\vec{z}\in W$. Then $\mathcal{P}\vec{z}=\vec{z}$ by Lemma~\ref{lma:KidentityonW} and $\vec{z}\in \mathcal{N}(I-\mathcal{P})$. Conversely, suppose $\mathcal{P}\vec{z}=\vec{z}$ for some $\vec{z}\in W\oplus U^s$. Then $\vec{z}=\vec{u}+\vec{v}$ for $\vec{u}\in W$ and $\vec{v}\in U^s$. Let $j$ be sufficiently large so that $\lVert \mathcal{P}^j|_{U^s}\rVert=\alpha<1$. Then
\begin{align*}
\lVert \mathcal{P}^j\vec{z}\rVert^2&=\lVert \mathcal{P}^j\vec{u}+\mathcal{P}^j\vec{v}\rVert^2\\
&\le\lVert \vec{u}\rVert^2+\alpha^2\lVert \vec{v}\rVert^2\\
&\le \lVert \vec{u}\rVert^2+\lVert \vec{v}\rVert^2\\
&=\lVert \vec{z}\rVert^2.\\
\end{align*}

Equality can only happen if $\vec{v}=0$. Therefore, $\vec{z}\in W$.
\end{proof}

\begin{lemma}
\label{lma:Kisprojection}
$\mathcal{P}^k$ restricted to $W\oplus U^s$ converges strongly, as $k\to\infty$, to the orthogonal projection onto $W$.
\end{lemma}

\begin{proof}
The proof is identical to that in \cite{Natterer2001}, using Lemmas~\ref{lma:sequence_zk_dags} and \ref{lma:nullspace_IminusK}.
\end{proof}

\begin{theorem}
If the system of equations given by $A\vec{x}=\vec{b}$ is consistent, then the sequence of estimates $\vec{x}_{r_i}^{(n)}$ converges to the solution $\vec{x}^M$ of minimal norm at all minimal nodes $r_i$, provided $\vec{x}^{(0)}\in U^s$.
\end{theorem}

\begin{proof}
Let $\vec{y}$ be any solution to the system of equations. For any $\vec{z}$,
\[
\mathcal{Q}\vec{z}=\vec{y}+\mathcal{P}(\vec{z}-\vec{y})
\]

By Lemma~\ref{lma:Kisprojection}, we have that for any $\vec{z}$,
\[
\mathcal{Q}^k\vec{z}\to \vec{y}+Pr(\vec{z}-\vec{y})
\]

as $k\to\infty$, where $Pr$ is the projection onto $W$. If $\vec{z}\in U^s$, we have that $\vec{y}+Pr(\vec{z}-\vec{y})$ is the unique solution to the system of equations that is in $W$, and hence the solution of minimal norm.
\end{proof}

\subsection{Inconsistent Systems}

Let there be $p$ paths from a minimal node to a maximal node, and enumerate these paths by $P_1,\dots,P_p$. For a given path $P_i$, an estimate will disperse from a minimal node $r_{P_i}$ to a maximal node $\ell_{P_i}$ through the vertices in the path $P_i$. For the series of projections along $P_i$, we can notate the update by
\begin{align*}
\vec{x}_{\ell_{P_i}}^{(n)}&=\mathcal{Q}_i\vec{x}_{r_{P_i}}^{(n)}\\
&=\left(I-\mathcal{S}_i^*(\mathcal{D}_i+\Omega_i\mathcal{L}_i)^{-1}\Omega_i\mathcal{S}_i\right)\vec{x}_{r_{P_i}}^{(n)}+\mathcal{S}_i^*(\mathcal{D}_i+\Omega_i\mathcal{L}_i)^{-1}\Omega_i\vec{b}_i\\
&=\mathcal{B}_i\vec{x}_{r_{P_i}}^{(n)}+\vec{\bm{\mathrm{b}}}_i.
\end{align*}

where $\mathcal{S}_i, \mathcal{D}_i,\mathcal{L}_i,$ and $\Omega_i$ are defined the same as before, based on the equations along the path $P_i$.

After the pooling stage, the estimate at each minimal node $r_i$ will be a weighted average of the estimates at all the maximal nodes. That is,
\begin{align*}
\vec{x}^{(n)}&=\begin{pmatrix}\left(\vec{x}_{r_1}^{(n)}\right)^T&\cdots&\left(\vec{x}_{r_s}^{(n)}\right)^T\end{pmatrix}^T,\\
\vec{x}_{r_i}^{(n+1)}&=\mathcal{Q}_{r_i}\vec{x}^{(n)}\\
&=\mathcal{B}_{r_i}\vec{x}^{(n)}+\vec{\bm{\mathrm{b}}}_{r_i}\\
&=w_{i,1}\mathcal{Q}_1\vec{x}_{r_{P_1}}^{(n)}+\cdots+w_{i,p}\mathcal{Q}_p\vec{x}_{r_{P_p}}^{(n)},\\
\vec{x}^{(n+1)}&=\begin{pmatrix}\left(\mathcal{Q}_{r_1}\vec{x}_{r_1}\right)^T&\cdots&\left(\mathcal{Q}_{r_s}\vec{x}_{r_s}\right)^T\end{pmatrix}^T
\end{align*}

where $w_{i,1}+\cdots+w_{i,p}=1$ and $w_{i,j}\ne 0$ whenever $r_i\preceq \ell_{P_j}$.

\begin{lemma}
$\mathcal{Q}$, and consequently $\mathcal{B}$, are Lipscshitz continuous with constant at most $1$.
\end{lemma}

\begin{proof}
$\mathcal{Q}$ is a convex combination of the operators $\mathcal{Q}_i$, each of which is Lipschitz continuous with constant at most $1$.
\end{proof}

Let $\hat{\mathcal{B}}$ be the restriction of $\mathcal{B}$ to the subspace $U^s$.

\begin{theorem}
The spectral radius of $\hat{\mathcal{B}}$ is less than $1$.
\end{theorem}

\begin{proof}
The proof is similar to that of Theorem 11 in REF.
\end{proof}

\begin{corollary}
For any initial input $\vec{x}^{(0)}\in U^s$, we have that the sequence given by
\[
\vec{x}^{(n+1)}=\hat{\mathcal{B}}\vec{x}^{(n)}+\vec{\bm{\mathrm{b}}}
\]

converges to a unique point in $U^s$, independent of $\vec{x}^{(0)}$, and the convergence rate is linear.
\end{corollary}

Define the following block matrices. The matrices $\mathcal{S},\mathcal{D},\mathcal{L}$, and $\Omega^{\vec{\omega}}$ contain $s$ copies of the matrices $\mathcal{S}',\mathcal{D}',\mathcal{L}'$, and $\Omega'$, respectively.
\begin{align*}
\mathcal{S}'&=(\mathcal{S}_1^T,\dots,\mathcal{S}_p^T)^T&\mathcal{S}&=\mathrm{diag}(\mathcal{S}',\dots,\mathcal{S}')\\
\mathcal{D}'&=\mathrm{diag}(\mathcal{D}_1,\dots,\mathcal{D}_p)&\mathcal{D}&=\mathrm{diag}(\mathcal{D}',\dots,\mathcal{D}')\\
\mathcal{L}'&=\mathrm{diag}(\mathcal{L}_1,\dots,\mathcal{L}_p)&\mathcal{L}&=\mathrm{diag}(\mathcal{L}',\dots,\mathcal{L}')\\
\Omega'&=\mathrm{diag}(\Omega_1,\dots,\Omega_p)&\Omega^{\vec{\omega}}&=\mathrm{diag}(\Omega',\dots,\Omega')\\
\mathcal{W}_i&=\mathrm{diag}(w_{i,1}I,\dots,w_{i,p}I)&\mathcal{W}&=\mathrm{diag}(\mathcal{W}_1,\dots,\mathcal{W}_s)
\end{align*}

Note that $\mathcal{W}$ commutes with $\mathcal{D}+\omega \mathcal{L}$. Then we rewrite an iteration as
\begin{align*}
\vec{x}^{(n+1)}&=\mathcal{Q}\vec{x}^{(n)}\\
&=\mathcal{B}\vec{x}^{(n)}+\vec{\bm{\mathrm{b}}}\\
&=\left(I-\mathcal{S}^*(\mathcal{D}+\Omega^{\vec{\omega}} \mathcal{L})^{-1}\Omega^{\vec{\omega}} \mathcal{W}\mathcal{S}\right)\vec{x}^{(n)}+\mathcal{S}^*(
\mathcal{D}+\Omega^{\vec{\omega}} \mathcal{L})^{-1}\Omega^{\vec{\omega}} \mathcal{W}\vec{b}
\end{align*}

\begin{lemma}
Let
\[
\vec{x}(\vec{\omega})=\lim_{n\to\infty}\vec{x}^{(n)}
\]

when the limit exists. Then $\vec{x}(\vec{\omega})$ is the unique vector that satisfies the conditions
\[
\mathcal{S}^*(\mathcal{D}+\Omega^{\vec{\omega}}\mathcal{L})^{-1}\Omega^{\vec{\omega}} \mathcal{W}(\vec{\bm{\mathrm{b}}}-\mathcal{S}\vec{z})=0;\quad \vec{z}\in U^s.
\]
\end{lemma}

\begin{proof}

\end{proof}

\begin{theorem}
For any positive vector $\vec{c}$ we have
\[
\lim_{\omega\to 0}\vec{x}(\omega \vec{c})=\vec{x}^{LS}
\]

where $\vec{x}^{LS}$ is the unique minimizer in $U^s$ of the functional
\[
\vec{z}\mapsto \langle \mathcal{D}^{-1}\mathcal{C} \mathcal{W}(\bm{\vec{\mathrm{b}}}-\mathcal{S}\vec{z}),(\bm{\vec{\mathrm{b}}}-\mathcal{S}\vec{z})\rangle,
\]

where $\mathcal{C}=\frac{1}{\omega}\Omega^{\omega \vec{c}}$.
\end{theorem}

\begin{proof}

\end{proof}


==> FutureDirection.tex <==
\section{Future Directions}


==> citations.tex <==
\cite{needell2014paved}
\cite{needell2015randomized}
\cite{necoara2019faster}
\cite{censor2001component}
\cite{chen2018kaczmarz}
\cite{cimmino1938calcolo}
\cite{kamath2015distributed}
\cite{liu2014asynchronous}
\cite{SV-09a}
